On compact packings of the plane with circles of three radii

A compact circle-packing $P$ of the Euclidean plane is a set of circles which bound mutually disjoint open discs with the property that, for every circle $S\in P$, there exists a maximal indexed set $\{A_{0},\ldots,A_{n-1}\}\subseteq P$ so that, for every $i\in\{0,\ldots,n-1\}$, the circle $A_{i}$ is tangent to both circles $S$ and $A_{i+1\mod n}.$ We show that there exist at most $13617$ pairs $(r,s)$ with $0<s<r<1$ for which there exist a compact circle-packing of the plane consisting of circles with radii $s$, $r$ and $1$. We discuss computing the exact values of such $0<s<r<1$ as roots of polynomials and exhibit a selection of compact circle-packings consisting of circles of three radii. We also discuss the apparent infeasibility of computing \emph{all} these values on contemporary consumer hardware with the methods employed in this paper.

==> base_definitions.tex <==
\global\long\def\norm#1{\left\Vert #1\right\Vert }

\global\long\def\abs#1{\left|#1\right|}

\global\long\def\set#1#2{\left\{  \vphantom{#1}\vphantom{#2}#1\right.\left|\ #2\vphantom{#1}\vphantom{#2}\right\}  }

\global\long\def\sphere#1{\mathbf{S}_{#1}}

\global\long\def\closedball#1{\mathbf{B}_{#1}}

\global\long\def\openball#1{\mathbb{B}_{#1}}

\global\long\def\duality#1#2{\left\langle \vphantom{#1}\vphantom{#2}#1\right.\left|\ #2\vphantom{#1}\vphantom{#2}\right\rangle }

\global\long\def\parenth#1{\left(#1\right)}

\global\long\def\curly#1{\left\{  #1\right\}  }

\global\long\def\blockbraces#1{\left[#1\right] }

\global\long\def\span{\textup{span}}

\global\long\def\image{\textup{Im}}

\textbf{}\global\long\def\support{\textup{supp}}

\global\long\def\N{\mathbb{N}}

\global\long\def\R{\mathbb{R}}

\global\long\def\Q{\mathbb{Q}}

\global\long\def\Rnonneg{\mathbb{R}_{\geq0}}

\global\long\def\C{\mathbb{C}}

\global\long\def\tocorr{\mathbb{\ \twoheadrightarrow\ }}

\global\long\def\restrict#1#2{#1|_{#2}}

\global\long\def\cal#1{\mathcal{#1}}


